Bounded and Divergent Trajectories And Expanding Curves on Homogeneous Spaces

Suppose $g_t$ is a $1$-parameter $\mathrm{Ad}$-diagonalizable subgroup of a Lie group $G$ and $\Gamma < G$ is a lattice. We study the dimension of bounded and divergent orbits of $g_t$ emanating from a class of curves lying on leaves of the unstable foliation of $g_t$ on the homogeneous space $G/\Gamma$. We obtain sharp upper bounds on the Hausdorff dimension of divergent on average orbits and show that the set of bounded orbits is winning in the sense of Schmidt (and, hence, has full dimension). The class of curves we study is roughly characterized by being tangent to copies of $\mathrm{SL}(2,\mathbb{R})$ inside $G$, which are not contained in a proper parabolic subgroup of $G$. We describe applications of our results to problems in Diophantine approximation by number fields and intrinsic Diophantine approximation on spheres. Our methods also yield the following result for lines in the space of square systems of linear forms: suppose $\varphi(s) = sY + Z$ where $Y\in \mathrm{GL}(n,\mathbb{R})$ and $Z\in M_{n,n}(\mathbb{R})$. Then, the dimension of the set of points $s$ such that $\varphi(s)$ is singular is at most $1/2$ while badly approximable points have Hausdorff dimension equal to $1$.

==> HeightLinearForms/weights.tex <==
\subsection{Preliminaries from representation theory}
	In this subsection, we recall some facts from the representation theory of semisimple Lie groups and set some notation that we will need later.
    
    Suppose $G$ is a semisimple algebraic Lie group and $A$ is a maximal abelian $\R$ diagonalizable subgroup of $G$.
    Denote by $P$ the set of algebraic characters on $\mf{a}$.
    
    Let $\Sigma \subset P $ denote the set of (restricted) roots of $A$ in the adjoint representation on the Lie algebra of $G$ which we denote by $\mf{h}$.
    The kernels of the linear functionals in $\Sigma$ divide $\mf{a}$ into cones called Weyl Chamber.
    We choose $\mc{C}$ to be one such closed Weyl chamber.
    Let $\Sigma^+ \subset \Sigma$ denote a set of positive roots relative to $\mc{C}$.
    That is
    \[ \Sigma^+ = \set{ \chi \in \Sigma: \chi (X) \geqslant 0 \text{ for all } X \in \mc{C} } \]
    Then, $\Sigma^+$ induces a partial order on $P$ as follows
    \begin{equation} \label{partial order weights}
    \l \leq \eta \Leftrightarrow \eta - \l \in \Sigma^+ 
    \end{equation} 
    
    Suppose $W$ is a finite dimensional vector space and $\rho: G \r \mrm{GL}(W)$ is an irreducible algebraic representation of $G$.
    For $\l \in P$, we denote by $W_\l$ the following subspace
    \begin{equation*}
    W_\l = \set{ w\in W: \rho( \exp( a)) w = \exp(\l(a)) w \text{ for all } a \in \mf{a}  }
    \end{equation*}
    Then, $W_\l$ is a weight space with weight $\l$.
    Since $A$ is abelian, we have
    \begin{equation*}
    W = \bigoplus_\l W_\l
    \end{equation*}
    The restricted weights of $\rho$ are weights $\l$ for which $W_\l \neq \set{0}$.
    
    Since $G$ is semisimple, the set of restricted weights of $\rho$ contains a unique maximal element with respect to the partial order~\eqref{partial order weights}.
    Such maximal weight is referred to as the highest weight of $\rho$.
    We denote by $P^+$ the subset of $P$ of all linear functionals which occur as highest weights in some irreducible representation of $G$.
    
    Given an arbitrary finite dimensional representation $V$ of $G$ and $\l\in P^+$, we use $V^\l$ to denote the direct sum of all irreducible subrepresentations of $V$ whose highest weight is $\l$.
    We denote by $\pi_\l:V \r V^\l$ the associated $G$-equivariant projection.
    
    
   
    
    
    
    
    
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     
     
     
    
    
    
    
    
    
    
    
    
    
    
    
    
